LLM-Enhanced Software Patch Localization

Open source software (OSS) is integral to modern product development, and any vulnerability within it potentially compromises numerous products. While developers strive to apply security patches, pinpointing these patches among extensive OSS updates remains a challenge. Security patch localization (SPL) recommendation methods are leading approaches to address this. However, existing SPL models often falter when a commit lacks a clear association with its corresponding CVE, and do not consider a scenario that a vulnerability has multiple patches proposed over time before it has been fully resolved. To address these challenges, we introduce LLM-SPL, a recommendation-based SPL approach that leverages the capabilities of the Large Language Model (LLM) to locate the security patch commit for a given CVE. More specifically, we propose a joint learning framework, in which the outputs of LLM serves as additional features to aid our recommendation model in prioritizing security patches. Our evaluation on a dataset of 1,915 CVEs associated with 2,461 patches demonstrates that LLM-SPL excels in ranking patch commits, surpassing the state-of-the-art method in terms of Recall, while significantly reducing manual effort. Notably, for vulnerabilities requiring multiple patches, LLM-SPL significantly improves Recall by 22.83\%, NDCG by 19.41\%, and reduces manual effort by over 25\% when checking up to the top 10 rankings. The dataset and source code are available at \url{https://anonymous.4open.science/r/LLM-SPL-91F8}.

==> 7_discuss.tex <==
\section{Discussion}

\noindent\textbf{Employing GPT-3.5}.
We employed GPT-3.5 to provide feedback for recommendations.
While GPT-3.5 is effective, there are other LLMs that also showcase robust performance in broad tasks. However, in our primary experiments, we found that explanations generated by GPT-3.5 regarding why a commit patches a specific CVE were of superior quality compared to those generated by other LLMs, including LLama~\cite{touvron2023llama}, Falcon-40B~\cite{falcon40b}, and Vicuna-13B~\cite{vicuna2023}. These results steered us towards the adoption of GPT-3.5. 
Incorporating a more advanced LLM might further enhance SPL performance.

\noindent\textbf{Fine-tuning LLM}.
We strategically utilize the outputs generated by a general-purpose LLM, GPT-3.5, instead of an LLM that's been fine-tuned specifically for our task. The challenges of using an LLM tailored for SPL stem from constrained computing resources and data availability. With our dataset of 11,802 gathered CVEs, attempting to fine-tune an LLM with tens of billions of parameters risks profound overfitting. While few-shot learning emerges as a potential solution, it warrants further studies.



\noindent\textbf{Limitation and future work}.
A limitation in our study arises when analyzing extremely large commits. Some of these commits can contain tens of thousands of tokens. In such cases, we truncate the commit content beyond 4097 tokens to adhere to GPT-3.5's input constraints. This truncation might inadvertently omit crucial information, leading these large commits to be ranked lower,  despite them being genuine patches for a CVE. Utilizing information extraction techniques that distill essential content from extensive commits into a limited number of tokens could alleviate this issue. This is one of our future works.



==> Table/3_challenge_code_diff.tex <==
\begin{table}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.05}
    \vspace{20pt}
    \caption{Information categories within commit code diff.}
    \label{table: information categories within commit code diff}  
    \footnotesize
    %\begin{adjustbox}{width=0.3\textwidth}

\begin{tabular}{|c|cc|}
\hline
\textbf{Component} & \multicolumn{2}{c|}{\textbf{Category}}                      \\ \hline
Comment            & \multicolumn{1}{c|}{Program functionality} & Modification reason \\ \hline
Source code        & \multicolumn{1}{c|}{Program functionality} & Modification location   \\ \hline
\end{tabular}
    

    %\end{adjustbox}
    
    
\end{table}

==> Table/4_LLM_confusion_matix.tex <==
\begin{table}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.05}
    \vspace{20pt}
    \caption{Confusion matrix for LLM's determination.}
    \label{table: Confusion matrix for LLM's identification}
    \footnotesize
    
\begin{tabular}{|cc|cc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}}                                    & \multicolumn{2}{c|}{\textbf{LLM Predicted}}                \\ \cline{3-4} 
\multicolumn{2}{|c|}{}                                                     & \multicolumn{1}{c|}{\textbf{Positive}} & \textbf{Negative} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Actual}}} & \textbf{Positive} & \multicolumn{1}{c|}{2,141}             & \textcolor{magenta}{320}            \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                 & \textbf{Negative} & \multicolumn{1}{c|}{\textcolor{magenta}{12,437}}               & 80,852            \\ \hline
\end{tabular}
\end{table}



==> Table/6_evaluation_1_1_Ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Data  & Model     & R@5    & R@10  & R@15 & NDCG@5 & NDCG@10          & NDCG@15 & $\text{R}_\text{CVE}$@5        & $\text{R}_\text{CVE}$@10        & $\text{R}_\text{CVE}$@15 \\ \hline

\multirow{3}{*}{1-1} & VCMatch(f0) & 91.67\% & 94.25\%   & 95.24\%         & 86.16\%   & 87.00\%          & 87.32\%                      & 91.67\%          & 94.25\%          & 95.24\%                        \\ \cline{2-11} 

& VCMatch(f0) + f1      & 92.59\% & 94.31\% & 95.37\%                   & 87.17\%                     & 87.73\%          & 88.01\%                      & 92.59\%          & 94.58\%          & 95.37\%                        \\ \cline{2-11} 


& VCMatch(f0) + f1 + f2 & \textbf{92.86\%} & \textbf{94.97\%} & \textbf{95.70\%}          & \textbf{87.60\%}            & \textbf{88.30\%} & \textbf{88.49\%}             & \textbf{92.86\%} & \textbf{94.97\%} & \textbf{95.70\%}               \\ \hline
\end{tabular}
\caption{Ablation Study on 1-1 Data}
\label{Ablation }
\end{table*}

==> Table/6_evaluation_Ablation_Study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{DATA} & \textbf{MODEL}  & \textbf{R@5}  & \textbf{R@10} & \textbf{R@15} & \textbf{NDCG@5} & \textbf{NDCG@10}  & \textbf{NDCG@15} & \textbf{$\text{R}_\text{CVE}$@5} & \textbf{$\text{R}_\text{CVE}$@10}        &\textbf{$\text{R}_\text{CVE}$@15} \\ \hline

\multirow{3}{*}{\textbf{FULL DATA}} & VCMatch($F_0$)           & 85.04\%          & 89.33\%          & 91.18\%                   & 79.94\%                     & 81.52\%          & 82.10\%                      & 82.45\%          & 87.10\%          & 89.03\%                        \\ \cline{2-11} 

& VCMatch($F_0$)+$F_1$      & 90.27\%          & 93.30\%          & 94.85\%                   & 84.44\%                     & 85.53\%          & 86.05\%                      & 87.46\%          & 91.07\%          & 93.11\%                        \\ \cline{2-11} 

& VCMatch($F_0$)+$F_1$+$F_2$ & \textbf{90.43\%} & \textbf{94.05\%} & \textbf{95.16\%}          & \textbf{84.99\%}            & \textbf{86.34\%} & \textbf{86.66\%}             & \textbf{87.51\%} & \textbf{92.42\%} & \textbf{93.83\%}               \\ \hline

\multirow{3}{*}{\textbf{1-1}}                       & VCMatch($F_0$)           & 91.67\%          & 94.25\%          & 95.24\%  & 86.16\%                     & 87.00\%          & 87.32\% & 91.67\%  & 94.25\% & 95.24\% \\ \cline{2-11}

& VCMatch($F_0$)+$F_1$ & 93.25\% & 95.03\% & 95.89\% & 87.17\%  & 87.73\% & 88.01\%  & 93.25\% & 95.03\% & 95.89\%\ \\ \cline{2-11} 
                                           
& VCMatch($F_0$)+$F_1$+$F_2$ & \textbf{93.45\%} & \textbf{95.10\%} & \textbf{96.16\%} & \textbf{88.08\%}            & \textbf{88.61\%} & \textbf{88.89\%}             & \textbf{93.45\%} & \textbf{95.10\%} & \textbf{96.16\%}               \\ \hline


{\multirow{3}{*}{\textbf{1-N}}} & VCMatch($F_0$)           & 60.18\%          & 70.89\%          & 75.19\%                   & 56.60\%                     & 60.99\%          & 62.52\%                      & 47.89\%          & 60.30\%          & 65.01\%                        \\ \cline{2-11} 
\multicolumn{1}{|l|}{}                     & VCMatch($F_0$)+$F_1$      & 79.10\%          & 86.81\%          & 90.93\%                   & \textbf{74.19\%}            & 77.30\%          & 78.29\%                      & 65.26\%          & 76.18\%          & 82.63\%                        \\ \cline{2-11} 
\multicolumn{1}{|l|}{}                     & VCMatch($F_0$)+$F_1$+$F_2$ & \textbf{79.64\%} & \textbf{90.11\%} & \textbf{91.42\%}          & 73.39\%                     & \textbf{78.11\%} & \textbf{78.70\%}             & \textbf{65.76\%} & \textbf{82.38\%} & \textbf{85.11\%}               \\ \hline
\end{tabular}
\caption{Ablation Study}
\label{table: Ablation Study}
\end{table*}








==> Table/6_evaluation_Experiment_Result.tex <==
\begin{table*}[]
% \renewcommand{\arraystretch}{1.2}
% \renewcommand\cellalign{l}
\renewcommand\cellset{\linespread{1.2}\selectfont}


\caption{Comparative Performance Metrics of Different Models with and without Graph Integration and GPT Feedback.}
\label{table: Model Result} 
\centering
\footnotesize
\begin{tabular}{cccccccc}
\hline

{Method} & Model & R@5 & R@10 & NDCG@5 & NDCG@10 & CVEs Find & CVEs Find\% \\ \hline

\multirow{3}{*}{\parbox{3cm}{No GPT-Feedback,\\No Graph}} 

& Wide\&Deep & 60.54\% & 70.53\% & 57.31\& & 61.46\% & 240 & 59.55\% \\ 

& XGBoost & 62.91\% & 70.09\% & 58.96\% & 61.93\% & 241 & 59.80\% \\ 

& VCMatch & 60.18\% & 70.89\% & 56.62\% &60.99\% & 243 & 60.29\% \\  \hline

\multirow{3}{*}{\parbox{3cm}{No GPT-Feedback\\+Raw Graph}}
& & & & & & &\\
& Wide\&Deep+Graph & 62.24\% & 73.42\% & 57.57\% & 62.23\% & 252 & 62.53\% \\ 
& & & & & & & \\
\hline

% \makecell[cl]{No GPT-feedback\\+Raw Graph}
% & Wide\&Deep+Graph & 62.24\% & 73.42\% & 57.57\% & 62.23\% & 252 & 62.53\% \\ \hline

% \multirow{3}[*]{}{}

\multirow{3}{*}{\parbox{3cm}{GPT-Relevance\\Feedback}}
& Wide\&Deep & 77.72\% & 88.36\% & 71.33\% & 75.66\% & 320 & 79.40\% \\ 

& XGBoost & 78.67\% & 87.11\% & 73.90\% & 77.28\% & 314 & 77.92\% \\

& VCMatch & 79.10\% & 86.81\% & \textbf{74.19\%} & 77.30\% & 307 & 76.18\% \\  \hline

\multirow{3}{*}{\parbox{3cm}{GPT-Relevance\\Feedback+GPT\\Connectivity Feedback}}
& & & & & & & \\
& Wide\&Deep+Graph & \textbf{79.62\%} & \textbf{89.71\%} & 74.09\% & \textbf{78.11\%} & \textbf{332} & \textbf{82.38\%} \\
& & & & & & & \\ \hline

% \makecell[cl]{GPT-Relevance\\Feedback+GPT\\Connectivity Feedback}
% & Wide\&Deep+Graph & \textbf{79.62\%} & \textbf{89.71\%} & 74.09\% & \textbf{78.11\%} & \textbf{332} & \textbf{82.38\%} \\ \hline

\end{tabular}
\end{table*}
\renewcommand{\arraystretch}{1}

==> Table/6_evaluation_Full_Dataset_Experiment_Result_.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\footnotesize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{DATA}} & \textbf{MODEL} & \textbf{R@5} & \textbf{R@10} & \textbf{R@15} & \textbf{NDCG@5} & \textbf{NDCG@10} & \textbf{NDCG@15} & \textbf{$\text{R}_\text{CVE}$@5}  & \textbf{$\text{R}_\text{CVE}$@10}        & \textbf{$\text{R}_\text{CVE}$@15} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Full Data}}} & VCMatch & 85.04\%          & 89.33\%          & 91.18\% & 79.94\%                     & 81.52\% & 82.10\%                      & 82.45\%          & 87.10\% & 89.03\%                        \\ \cline{2-11} 
\multicolumn{1}{|c|}{} & LLM-SPL & \textbf{90.43\%} & \textbf{94.05\%} & \textbf{95.16\%}  & \textbf{84.99\%} & \textbf{86.34\%} & \textbf{86.66\%}             & \textbf{87.51\%} & \textbf{92.42\%} & \textbf{93.83\%}               \\ \hline

\multirow{2}{1cm}{\centering \textbf{1-1}}& VCMatch & 91.67\%          & 94.25\%          & 95.24\%                   & 86.16\%                     & 87.00\%          & 87.32\%                      & 91.67\%          & 94.25\%          & 95.24\%                        \\ \cline{2-11} 
                                                 & LLM-SPL & \textbf{93.45\%} & \textbf{95.10\%} & \textbf{96.16\%}          & \textbf{88.08\%}            & \textbf{88.61\%} & \textbf{88.89\%}             & \textbf{93.45\%} & \textbf{95.10\%} & \textbf{96.16\%}               \\ \hline
\multirow{2}{1cm}{\centering \textbf{1-N}}                             & VCMatch & 60.18\%          & 70.89\%          & 75.19\%                   & 56.60\%                     & 60.99\%          & 62.52\%                      & 47.89\%          & 60.30\%          & 65.01\%                        \\ \cline{2-11} 
                                                 & LLM-SPL & \textbf{79.64\%} & \textbf{90.11\%} & \textbf{91.42\%}          & \textbf{73.39\%}            & \textbf{78.11\%} & \textbf{78.70\%}             & \textbf{65.76\%} & \textbf{82.38\%} & \textbf{85.11\%}               \\ \hline
\end{tabular}
    \caption{Performance comparison of the VCMatch and LLM-SPL models for security patch localization}
    \label{table: Full Dataset Result}
\end{table*}







% \begin{table*}[t]
%     \centering
%     \begin{tabular}{lccccccccc} 
%     \toprule


%     % \multirow{2}{*}{Model} & \multicolumn{3}{c}{Full Dataset} & \multicolumn{3}{c}{1-to-1} & \multicolumn{3}{c}{1-to-N} \\
%     \multirow{2}{*}{Model} & \multicolumn{3}{>{\centering\arraybackslash}p{4.3cm}}{Full Dataset}
%  & \multicolumn{3}{>{\centering\arraybackslash}p{4.2cm}}{1-to-1} & \multicolumn{3}{>{\centering\arraybackslash}p{4.2cm}}{1-to-N} \\
%     % \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}    
%     & Recall & NDCG & $\text{Recall}_\text{CVE}$ & Recall & NDCG & $\text{Recall}_\text{CVE}$ & Recall & NDCG & $\text{Recall}_{\text{CVE}}$  \\ 
    
%     \midrule
%     % \noalign{\smallskip}
%     VCMatch & 89.33\% & 81.52\% & 87.10\% & 94.25\% & 87.00\% & 94.25\% & 70.89\% & 60.98\% & 60.29\% \\
%     \noalign{\smallskip}
%     LLM-SPL & \textbf{93.95\%} & \textbf{86.09\%} & \textbf{92.32\%} & \textbf{94.97\%} & \textbf{88.30\%} & \textbf{94.97\%} & \textbf{89.71\%} & \textbf{78.11\%} & \textbf{82.38\%}   \\
%     \bottomrule
%     \end{tabular}
%     \caption{Performance comparison of the VCMatch and LLM-SPL models for security patch localization}
%     \label{table: Full Dataset Result}
% \end{table*}

==> Table/6_evaluation_Mixed_CVE_Level_Experiment_Result.tex <==
% 这个里面的各个模块的名字还需要改动
\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\caption{CVE Level Performance Comparison On 2-Step Feedback on Mixed Dataset}
\label{table: Mixed CVE Level Model Result} 
\centering
\footnotesize
\begin{tabular}{ccccccc}
\hline
Model & Recall @5 & Recall @10 & NDCG@5 & NDCG@10 & CVEs Find & CVEs Find\% \\ \hline

VCMatch(baseline) & 85.04\% & 89.33\% & 79.94\% & 81.52\%  & 1668 & 87.10\% \\ 

VCMatch+GPT Graph & 87.20\% & 91.33\% & 81.91\% & 83.47\% & 1720 & 89.82\% \\

VCMatch+GPT Feature & 89.75\% & 92.73\% & 84.44\% & 85.53\% & 1733 & 90.50\% \\ 

VCMatch+GPT Feature+GPT Graph & \textbf{89.96\%} &\textbf{94.13}\% & \textbf{84.72\%} & \textbf{86.09\%} & \textbf{1768} & \textbf{92.32\%} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{table*}

==> Table/6_evaluation_Mixed_Commit_Level_Experiment_Result.tex <==
% 这个里面的各个模块的名字还需要改动
\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\caption{Commit Level Performance Comparison On 2-Step Feedback on Mixed Dataset}
\label{table: Mixed CVE Level Model Result} 
\centering
\footnotesize
\begin{tabular}{ccccc}
\hline
Model & Recall @5 & Recall @10 &  \# Commits Retrieve in top5 & \# Commits Retrieve in top 10\\ \hline

VCMatch(baseline) & 78.50\% & 84.80\% & 1932 & 2087 \\ 

VCMatch+GPT Graph & 81.55\% & 88.05\% & 2007 & 2167 \\

VCMatch+GPT Feature & 86.67\% & 91.30\% & 2133 & 2247 \\

VCMatch+GPT Feature+GPT Graph & \textbf{86.75\%} &\textbf{92.77}\% & \textbf{2135} & \textbf{2283} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{table*}

==> Table/6_evaluation_Multi_CVE_Level_Experiment_Result.tex <==
% 这个里面的各个模块的名字还需要改动
\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\caption{CVE-Level Performance Comparison On 2-Step Feedback on Multi-Patches Dataset}
\label{table: Multi CVE Level Model Result } 
\centering
\footnotesize
\begin{tabular}{ccccccc}
\hline
Model & Recall @5 & Recall @10 & NDCG@5 & NDCG@10 & CVEs Find & CVEs Find\% \\ \hline
VCMatch(baseline) & 60.18\% & 70.89\% & 56.60\% & 60.99\%  & 243 & 60.29\% \\ 
VCMatch+GPT Graph & 64.97\% & 77.68\% & 59.98\% & 65.13\% & 284 & 70.47\% \\
VCMatch+GPT Feature & 79.10\% & 86.81\% & \textbf{74.19\%} & 77.30\% & 307 & 76.18\% \\ 
VCMatch+GPT Feature+GPT Graph & \textbf{79.64\%} &\textbf{89.71}\% & 74.09\% & \textbf{78.11\%} & \textbf{332} & \textbf{82.38\%} \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{table*}

==> Table/6_evaluation_ablation_r_cve.tex <==
\begin{table*}[]
    \centering    
    \caption{Result of ablation study on Recall$_{CVE}$ ($R_{CVE}@k$)}
    \label{table: result of ablation study on recall cve}
    \begin{adjustbox}{width=1\textwidth}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Data}          & \textbf{Feature} & \textbf{1}                     & \textbf{2}                     & \textbf{3}                     & \textbf{4}                     & \textbf{5}                     & \textbf{6}                     & \textbf{7}                     & \textbf{8}                     & \textbf{9}                     & \textbf{10}                    \\ \hline
                       & F0               & 62.14\%                        & 74.99\%                        & 78.49\%                        & 80.68\%                        & 82.45\%                        & 83.66\%                        & 84.75\%                        & 85.43\%                        & 86.27\%                        & 87.10\%                        \\ \cline{2-12} 
                       & F0+F1            & 63.13\%                        & 77.70\%                        & {\color[HTML]{3531FF} 82.87\%} & {\color[HTML]{3531FF} 85.54\%} & 86.95\%                        & 87.78\%                        & 88.62\%                        & 89.40\%                        & 89.97\%                        & 90.50\%                        \\ \cline{2-12} 
\multirow{-3}{*}{Full} & F0+F1+F2         & {\color[HTML]{3531FF} 64.07\%} & {\color[HTML]{3531FF} 77.81\%} & {\color[HTML]{3531FF} 82.87\%} & 85.33\%                        & {\color[HTML]{3531FF} 87.52\%} & {\color[HTML]{3531FF} 88.62\%} & {\color[HTML]{3531FF} 89.50\%} & {\color[HTML]{3531FF} 90.39\%} & {\color[HTML]{3531FF} 91.33\%} & {\color[HTML]{3531FF} 92.43\%} \\ \hline
                       & F0               & 78.70\%                        & 87.57\%                        & 89.55\%                        & 90.67\%                        & 91.67\%                        & 92.39\%                        & 93.12\%                        & 93.58\%                        & 93.98\%                        & 94.25\%                        \\ \cline{2-12} 
                       & F0+F1            & 79.96\%                        & 88.10\%                        & 90.61\%                        & 91.87\%                        & 92.59\%                        & 93.06\%                        & 93.39\%                        & 93.85\%                        & 94.05\%                        & 94.31\%                        \\ \cline{2-12} 
\multirow{-3}{*}{1-1}  & F0+F1+F2         & {\color[HTML]{3531FF} 81.15\%} & {\color[HTML]{3531FF} 88.96\%} & {\color[HTML]{3531FF} 90.81\%} & {\color[HTML]{3531FF} 92.20\%} & {\color[HTML]{3531FF} 93.45\%} & {\color[HTML]{3531FF} 93.85\%} & {\color[HTML]{3531FF} 94.11\%} & {\color[HTML]{3531FF} 94.44\%} & {\color[HTML]{3531FF} 94.71\%} & {\color[HTML]{3531FF} 95.11\%} \\ \hline
                       & F0               & 0.00\%                         & 27.79\%                        & 36.97\%                        & 43.18\%                        & 47.89\%                        & 50.87\%                        & 53.35\%                        & 54.84\%                        & 57.32\%                        & 60.30\%                        \\ \cline{2-12} 
                       & F0+F1            & 0.00\%                         & {\color[HTML]{3531FF} 38.71\%} & {\color[HTML]{3531FF} 53.85\%} & {\color[HTML]{3531FF} 61.79\%} & 65.26\%                        & 67.99\%                        & 70.72\%                        & 72.70\%                        & 74.69\%                        & 76.18\%                        \\ \cline{2-12} 
\multirow{-3}{*}{1-N}  & F0+F1+F2         & 0.00\%                         & 35.98\%                        & 53.10\%                        & 59.55\%                        & {\color[HTML]{3531FF} 65.76\%} & {\color[HTML]{3531FF} 68.98\%} & {\color[HTML]{3531FF} 72.21\%} & {\color[HTML]{3531FF} 75.19\%} & {\color[HTML]{3531FF} 78.66\%} & {\color[HTML]{3531FF} 82.38\%} \\ \hline
\end{tabular}
    
    \end{adjustbox}
\end{table*}

==> Table/6_evaluation_other_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\footnotesize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{DATA}} & \textbf{MODEL} & \textbf{R@5} & \textbf{R@10} & \textbf{R@15} & \textbf{NDCG@5} & \textbf{NDCG@10} & \textbf{NDCG@15} & \textbf{$\text{R}_\text{CVE}$@5}  & \textbf{$\text{R}_\text{CVE}$@10}        & \textbf{$\text{R}_\text{CVE}$@15} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Full Data}}} & Wide\&Deep & 86.47\%          & 89.99\%          & 91.59\% & 81.47\%                     & 82.81\% & 83.31\%                      & 83.24\%          & 87.68\% & 89.35\%                        \\ \cline{2-11} 
\multicolumn{1}{|c|}{} & XGBoost & 86.19\% & 89.89\% & 91.98\%  & 80.66\% & 81.99\% & 82.65\%             &  83.55\% & 87.78\% & 89.97\%               \\ \hline

\multirow{2}{1cm}{\centering \textbf{1-1}}& Wide\&Deep & 93.39\%          & 95.17\%          & 96.10\%                   & 87.91\%                     & 88.50\%          & 88.74\%                      & 93.39\%          & 95.17\%          & 96.10\%                        \\ \cline{2-11} 

& XGBoost & 92.39\% & 95.17\% & 96.23\%          & 86.45\%           & 87.34\% & 87.62\%             & 92.39\% & 95.17\% & 96.23\%               \\ \hline
\multirow{2}{1cm}{\centering \textbf{1-N}}                             & Wide\&Deep & 60.54\%          & 70.53\%          & 74.69\%                   & 57.31\%                     & 61.46\%          & 62.91\%                      & 45.16\%          & 59.55\%          & 64.02\%                        \\ \cline{2-11} 

& XGBoost & 62.91\% & 70.09\% & 76.05\%       & 58.96\%            & 61.93\% & 64.01\%             & 50.37\% & 60.05\% & 66.50\%               \\ \hline
\end{tabular}
    % \caption{Performance comparison of the VCMatch and LLM-SPL models for security patch localization}
    \label{table: other Result}
\end{table*}







% \begin{table*}[t]
%     \centering
%     \begin{tabular}{lccccccccc} 
%     \toprule


%     % \multirow{2}{*}{Model} & \multicolumn{3}{c}{Full Dataset} & \multicolumn{3}{c}{1-to-1} & \multicolumn{3}{c}{1-to-N} \\
%     \multirow{2}{*}{Model} & \multicolumn{3}{>{\centering\arraybackslash}p{4.3cm}}{Full Dataset}
%  & \multicolumn{3}{>{\centering\arraybackslash}p{4.2cm}}{1-to-1} & \multicolumn{3}{>{\centering\arraybackslash}p{4.2cm}}{1-to-N} \\
%     % \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}    
%     & Recall & NDCG & $\text{Recall}_\text{CVE}$ & Recall & NDCG & $\text{Recall}_\text{CVE}$ & Recall & NDCG & $\text{Recall}_{\text{CVE}}$  \\ 
    
%     \midrule
%     % \noalign{\smallskip}
%     VCMatch & 89.33\% & 81.52\% & 87.10\% & 94.25\% & 87.00\% & 94.25\% & 70.89\% & 60.98\% & 60.29\% \\
%     \noalign{\smallskip}
%     LLM-SPL & \textbf{93.95\%} & \textbf{86.09\%} & \textbf{92.32\%} & \textbf{94.97\%} & \textbf{88.30\%} & \textbf{94.97\%} & \textbf{89.71\%} & \textbf{78.11\%} & \textbf{82.38\%}   \\
%     \bottomrule
%     \end{tabular}
%     \caption{Performance comparison of the VCMatch and LLM-SPL models for security patch localization}
%     \label{table: Full Dataset Result}
% \end{table*}\textbf{}

==> Table/6_evaluation_overall_labor_test_transposed.tex <==
\begin{table*}
    % \centering
    %\renewcommand{\arraystretch}{1.05}
    \caption{Manual Effort ($M@k$) of PatchScout, FixFinder, VCMatch, and LLM-SPL.}    
    \label{table: Manual Effort of models}
    \vspace{-2pt}
    \begin{adjustbox}{width=0.055\textwidth}
    % \small
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \textbf{Data} & \textbf{Model} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} \\ \hline
    \multirow{4}{*}{Full} 
    & PatchScout & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & FixFinder & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & VCMatch & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.63} & \multicolumn{1}{c|}{1.84} & \multicolumn{1}{c|}{2.04} & \multicolumn{1}{c|}{2.21} & \multicolumn{1}{c|}{2.38} & \multicolumn{1}{c|}{2.53} & \multicolumn{1}{c|}{2.67} & \multicolumn{1}{c|}{2.81} \\ \cline{2-13}
    & LLM-SPL & \multicolumn{1}{c|}{1.00 \teal{$=$}} & \multicolumn{1}{c|}{1.35 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.56 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.72 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.85 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.97 \blue{$\downarrow$}} & \multicolumn{1}{c|}{2.07 \blue{$\downarrow$}} & \multicolumn{1}{c|}{2.17 \blue{$\downarrow$}} & \multicolumn{1}{c|}{2.26 \blue{$\downarrow$}} & \multicolumn{1}{c|}{2.34 \blue{$\downarrow$}} \\ \hline
    \multirow{4}{*}{1-1} 
    & PatchScout & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & FixFinder & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & VCMatch & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{1.21} & \multicolumn{1}{c|}{1.34} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{1.69} & \multicolumn{1}{c|}{1.76} & \multicolumn{1}{c|}{1.83} & \multicolumn{1}{c|}{1.89} \\ \cline{2-13}
    & LLM-SPL & \multicolumn{1}{c|}{1.00 \teal{$=$}} & \multicolumn{1}{c|}{1.18 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.29 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.37 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.44 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.51 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.56 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.62 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.67 \blue{$\downarrow$}} & \multicolumn{1}{c|}{1.72 \blue{$\downarrow$}} \\ \hline
    \multirow{4}{*}{1-N} 
    & PatchScout & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & FixFinder & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} & \multicolumn{1}{c|}{xx.xx} \\ \cline{2-13}
    & VCMatch & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{2.00} & \multicolumn{1}{c|}{2.72} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.44} & \multicolumn{1}{c|}{4.93} & \multicolumn{1}{c|}{5.40} & \multicolumn{1}{c|}{5.85} & \multicolumn{1}{c|}{6.28} \\ \cline{2-13}
    & LLM-SPL & \multicolumn{1}{c|}{1.00 \teal{$=$}} & \multicolumn{1}{c|}{2.00 \teal{$=$}} & \multicolumn{1}{c|}{2.58 \blue{$\downarrow$}} & \multicolumn{1}{c|}{3.02 \blue{$\downarrow$}} & \multicolumn{1}{c|}{3.38 \blue{$\downarrow$}} & \multicolumn{1}{c|}{3.69 \blue{$\downarrow$}} & \multicolumn{1}{c|}{3.97 \blue{$\downarrow$}} & \multicolumn{1}{c|}{4.23 \blue{$\downarrow$}} & \multicolumn{1}{c|}{4.47 \blue{$\downarrow$}} & \multicolumn{1}{c|}{4.67 \blue{$\downarrow$}} \\ \hline
    \end{tabular}
    
    \end{adjustbox}
    \vspace{-10pt}
\end{table*}


==> backup.tex <==
urrent SPL techniques are based upon recommendation models, utilizing the content within CVEs and commits as the basis for model training, aiming to identify the commits that are most likely addressing the vulnerabilities specified in given CVEs.~\cite{XXX}
Consequently, the effectiveness of SPL is fundamentally dependent on the deep understanding of these contents and on the quality of the training dataset.
However, the content in CVEs and commits is often complex and intricate, and the available training dataset is noticeable sparse, thereby introducing two significant challenges in SPL.
Additionally, there are certain vulnerabilities that are addressed by multiple distinct patches over time before being fully resolved, a scenario inadequately handled by existing SPL works.
We believe that identifying relationships among commits and incorporating this information into model training could be potentially helpful. However, we found constructing these relationships is a challenging task.
In the following, we will elaborate on these three challenges to SPL.



Furthermore, even though the LLM achieved a commendable recall of 87\%, it unfortunately missed 320 commits.
To understand the reasons for these omissions, we conducted a study of 50 randomly sampled cases from this group.
What we observed was that the content of these overlooked commits indeed lack direct associations with the content of respective CVEs, which explains the failure in detection.
Notably, among these, a subset of \blue{949} commits collaborate with other specific commits to address the CVEs. And we found, for these pairs of commits, not only is the latter one already identified by the LLM, but the relationship between them is also established successfully by the LLM in our supplementary experiments.
This observation aligns with the 1-N scenario discussed in Section~\ref{subsec: Challenge 3: Establishment of Inter-commit Relationships}, implying that leveraging inter-commit relationships might be instrumental in rectifying these missed instances.
Moreover, given this observation, a natural question arises: Could we perhaps feed the LLM with a CVE alongside its multiple associated commits? The intention of this would be to see if the LLM would use the inter-commit information to deduce and then recover the previously missed commits.
However, this approach is not feasible in practice.
The reason lies in the architecture of the LLM itself: every interaction with the LLM has a certain length limitation, and each of these interactions is independent of the others~~\cite{}. For instance, in GPT-3.5 we used, the maximum token count for a prompt is 2,048 tokens~\cite{}. 
Given that commits are typically quite mainly long due to their code diffs, this makes it very difficult, if not impossible, to feed multiple, sometimes even just two, commits together into the LLM.


Furthermore, even though the LLM achieved a commendable recall of 87\%, it unfortunately missed 320 commits (false negatives).
To understand why this happened, we analyzed 50 samples randomly selected from these commits.
What we observed was that the content of these overlooked commits indeed lack direct associations with the content of respective CVEs, as exampled in Figure~\ref{figure: Example of weak relationship between commit and CVE}, which explains the failure in detection.
Notably, among these, a subset of XXX commits collaborate with other specific commits to address the CVEs. And we found, for these pairs of commits, not only is the latter one already identified by the LLM, but the relationship between them is also established successfully by the LLM in our supplementary experiments.
This observation aligns with the 1-N scenario discussed in Section~\ref{subsec: Challenge 3: Establishment of Inter-commit Relationships}, implying that leveraging inter-commit relationships might be instrumental in rectifying these missed instances.
Moreover, given this observation, a natural question arises: Could we perhaps feed the LLM with a CVE alongside its multiple associated commits? The intention of this would be to see if the LLM would use the inter-commit information to deduce and then recover the previously missed commits.
However, this approach is not feasible in practice.
The reason lies in the architecture of the LLM itself: every interaction with the LLM has a certain length limitation, and each of these interactions is independent of the others~~\cite{}. For instance, in GPT-3.5 we used, the maximum token count for a prompt is 2,048 tokens~\cite{}. 
Given that commits are typically quite mainly long due to their code diffs, this makes it very difficult, if not impossible, to feed multiple, sometimes even just two, commits together into the LLM.
